Deep Embedded K-Means Clustering

Recently, deep clustering methods have gained momentum because of the high representational power of deep neural networks (DNNs) such as autoencoder. The key idea is that representation learning and clustering can reinforce each other: Good representations lead to good clustering while good clustering provides good supervisory signals to representation learning. Critical questions include: 1) How to optimize representation learning and clustering? 2) Should the reconstruction loss of autoencoder be considered always? In this paper, we propose DEKM (for Deep Embedded K-Means) to answer these two questions. Since the embedding space generated by autoencoder may have no obvious cluster structures, we propose to further transform the embedding space to a new space that reveals the cluster-structure information. This is achieved by an orthonormal transformation matrix, which contains the eigenvectors of the within-class scatter matrix of K-means. The eigenvalues indicate the importance of the eigenvectors' contributions to the cluster-structure information in the new space. Our goal is to increase the cluster-structure information. To this end, we discard the decoder and propose a greedy method to optimize the representation. Representation learning and clustering are alternately optimized by DEKM. Experimental results on the real-world datasets demonstrate that DEKM achieves state-of-the-art performance.

==> sec_results.tex <==
\section{Experimental Results}
\subsection{Evaluation of Clustering Algorithm}
We run DeepKmeans on each dataset and report the average results over three times. Table~\ref{tab_all} reports the clustering performance of different methods on the aforementioned datasets in terms of normalized mutual information (NMI) and unsupervised clustering accuracy (ACC). For the comparison methods, we present the reported results from their original papers if they are available (marked by $^*$ in Table~\ref{tab_all}). For unreported results on specific datasets, we run the released code mentioned in the original papers. When the released code is not available or running the released code is not practical, we put dash marks (-) in Table~\ref{tab_all}. 

\begin{table*}[!htb]
	\caption{Clustering performance of different algorithms in terms of the unsupervised clustering accuracy (ACC\%) and normalized mutual information (NMI\%). These results marked by $^*$ come from the original papers. (-) denotes that the result is not available. }
	\begin{center}
		\begin{tabular}{|c|c|c|c|c|c|c|c|c|}
			\hline
			\multirow{2}{*}{Method} & \multicolumn{2}{c|}{MNIST}      & \multicolumn{2}{c|}{USPS}       & \multicolumn{2}{c|}{COIL-20}    & \multicolumn{2}{c|}{FRGC}       \\ \cline{2-9} 
			& ACC            & NMI            & ACC            & NMI            & ACC            & NMI            & ACC            & NMI            \\ \hline
			K-means                 & 53.4           & 50.0           & 66.81          & 62.62          & 25.28          & 67.17          & 12.63          & 18.27          \\ \hline
			PCA + K-means             & 53.13          & 49.91          & 54.2           & 60.96          & 26.53          & 65.34          & 12.55          & 15.19          \\ \hline
			ConvAE + K-means              & 85.47          & 80.53          & 74.84          & 74.16          & 68.82          & 79.56          & 33.31          & 42.81          \\ \hline
			DEC \cite{DEC_xie2016unsupervised}                     & 84.3$^*$          & 83.72$^*$         & 73.68$^*$         & 75.29$^*$         & 65.42$^*$         & 80.49$^*$         & 37.1$^*$          & 44.6$^*$          \\ \hline
%			DCEC \cite{DCEC_guo2017deep}                   & 87.16          & 85.92          & 78.35          & 81.34          & 71.88          & 82.24          & 33.4           & 41.5           \\ \hline
			IDEC \cite{IDEC_guo2017improved}                   & 88.06$^*$         & 86.72$^*$         & 76.05$^*$         & 78.46$^*$         & -              & -              & -              & -              \\ \hline
			DCN \cite{DCN_yang2017towards}                    & 84.0           & 80.0           & 67.0           & 67.0           & 74.0           & 81.0           & -           & -          \\ \hline
			DBC \cite{li2018discriminatively}                     & 96.4$^*$          & \textbf{91.7$^*$} & 74.3$^*$          & 72.4$^*$          & \textbf{79.3$^*$} & \textbf{89.5$^*$} & -              & -              \\ \hline
			DeepKmeans              & 95.75          & 91.06          & 79.75          & 82.23          & 69.03          & 80.06          & 38.59          & 50.78          \\ \hline
			DeepKmeans\_$l2$          & \textbf{96.57} & 91.61          & \textbf{92.97} & \textbf{85.01} & 75.07          & 82.55          & \textbf{41.47} & \textbf{55.56} \\ \hline
		\end{tabular}
		\label{tab_all}
	\end{center}
\end{table*}

According to Table~\ref{tab_all}, DeepKmeans outperforms the comparison methods on most of the datasets. It achieves competitive results to DBC on COIL-20. Especially, DeepKmeans outperforms all the comparison methods with a large margin on USPS. As we can see, all the deep clustering methods perform much better than the traditional shallow methods (i.e., K-means and K-means+PCA). This suggests that the embedding space generated by autoencoders is more advantageous for clustering. Both DeepKmeans and DCEC use the same architecture of autoencoder. The performance gap between DeepKmeans and DCEC reflects the effect of different clustering optimizing strategy. The clustering optimizing strategy of DeepKmeans is superior to that of DCEC.

\subsection{Adaptive Dimension Updating}

\subsubsection{Optimization Strategy Comparison}
To compare the efficiency of different optimizing strategies for refining clustering, we visualize the embedding representations during clustering optimizing proceeding. The samples comes from  a subset of MNIST dataset containing random 4 categories. We do not adopt the t-SNE \cite{van2009learning} projection of the high dimensional embedding representations into 2-D space for visualization. Instead, we just set the units of the embedding layer to 2. Then we use the two dimensions to span a visual 2-D space, which is in essence visualization of embedding space. We compare the clustering optimizing strategy of DeepKmeans’s adaptive dimension updating with the strategy of DEC’s auxiliary target distribution \cite{DEC_xie2016unsupervised}. 

Fig.~\ref{fig_2D} shows representations in the embedding space during clustering optimizing proceeding. According to Fig.~\ref{fig_2D}, from left to right in each row, as the optimization proceeds, DeepKmeans and DEC both gather samples into clusters by letting the samples get closer to their respective centroids. That is, both DeepKmeans and DEC are doing the same thing, reducing the inner-class distance of each cluster for discriminative embedding representations. Furthermore, comparing each column of Fig.~\ref{fig_2D}, we can see that DeepKmeans only optimizes along the direction of the black line (i.e., the direction of corresponding eigenvector of the biggest eigenvalue) than DEC's all directions. Such an indirect way to optimize can reduce the loyalty dependence of pseudo label during clustering optimizing. In addition, focusing on the curve of clustering performance during the optimizing proceeding in Fig.~\ref{fig_2D_ACC}, we can see that DeepKmeans having better clustering performance than DEC.

\begin{figure}[!htb]
	\centering
	\subfigure[ACC]{\includegraphics[width=0.24\textwidth]{img/2D_ACC.png}}  
	\subfigure[NMI]{\includegraphics[width=0.24\textwidth]{img/2D_NMI.png}} 
	\caption{The clustering performance of DEC and DeepKMeans as the clustering optimizing proceeds.}
	\label{fig_2D_ACC}
\end{figure}


Now, we intuitively illustrate why adaptive dimension updating is better. In the first column of Fig.~\ref{fig_2D}, some points in the intersection of green points and white points are misclassified by K-means. So the pseudo label served by those points for alternate optimizing is not faithful. It is not advisable that letting those points get closer to their respective centroids (the samples on each background block getting close to the black cross of that background block) along all directions. For DeepKmeans, we only let those samples get closer to their respective centroids along the black line. That is, we first project all samples and centroids to the black line and then let all samples get closer to respective centroids alone the line. Fortunately, for those misclassified samples, we can see that the centroids of green points and white points are close to each other along the black line. Although those misclassified points go close to the wrong centroid, the negative consequences of those wrong pseudo labels can be alleviated. On the DEC side, there is not corresponding mechanism.

\subsubsection{Dimension-based Updating Strategy}
Furthermore, we examine the effect of a variety of dimension-based updating strategies on MNIST dataset. Specifically, we compare the following strategies: updating the least important clustering dimension of $\rm{h}$ (i.e., the last dimension of ${\rm{h}_V}$), updating all dimension of ${\rm{h}_V}$, updating random one dimension of $\rm{h}$ each iteration, updating random one dimension of $\rm{h}_V$ every iteration, updating all dimension of $\rm{h}$ and the clustering optimizing strategy of DEC.
\label{sec_adaptiveDimensionUpdating}

According to Fig.~\ref{fig_ACC}, we can see that the strategy of updating the least important clustering dimension is indeed the best strategy among the tested. And compared with the counterpart one dimension updating strategy: updating the last dimension of $\rm{h}$, it is more desired. Comparing the brown curve with the purple, we can see that updating all dimension of ${\rm{h}_V}$ approximately equals to updating all dimension of $\rm{h}$, which also demonstrates performing K-means in the original input space equals to in the transformed space by $V$.

\begin{figure*}[!htb]
	\centering	
	\subfigure[Raw data]{\includegraphics[width=0.24\linewidth]{img/em_ori.png}}
	\subfigure[Raw data + PCA]{\includegraphics[width=0.24\linewidth]{img/em_pca.png}
		\label{em_pca}}
	\subfigure[ConvAE]{\includegraphics[width=0.24\linewidth]{img/em_ae.png}
		\label{em_ae}}
	\subfigure[ConvAE\_$l2$]{\includegraphics[width=0.24\linewidth]{img/em_ae_l2.png}
		\label{em_ae_l2}}
	
	\subfigure[DEC]{\includegraphics[width=0.24\linewidth]{img/em_DEC.png}
		\label{em_DEC}}
	\subfigure[DCEC]{\includegraphics[width=0.24\linewidth]{img/em_DCEC.png}
		\label{em_DCEC}}
	\subfigure[DeepKmeans]{\includegraphics[width=0.24\linewidth]{img/em_DK.png}
		\label{em_DK}}
	\subfigure[DeepKmeans\_$l2$]{\includegraphics[width=0.24\linewidth]{img/em_DK_l2.png}}	
	
	\caption{Visualization comparison of discrimination ability of embedding space of different algorithms on MNIST dataset.}
	\label{fig_em}
\end{figure*}

\begin{figure}[!htb]
	\centerline{\includegraphics{img/ACC}}
	\caption{The clustering performance of different dimension-based updating strategies as clustering optimizing proceeds on MNIST dataset.}
	\label{fig_ACC}
\end{figure}


\subsection{Embedding Space Comparison}
Fig.~\ref{fig_em} demonstrates the discrimination ability of DeepKmeans by comparing the embedding space of different algorithms on MNIST dataset using t-SNE. Fig.\ref{em_pca} denote perform t-SNE on the representations of PCA (variance that needs to be explained is greater than 90\%). Fig.~\ref{em_ae}, Fig.~\ref{em_ae_l2} denotes respectively the embedding space of DeepKmeans and DeepKmeans\_$l2$ without clustering optimizing. As shown, DeepKmeans provides a significantly more discriminative embedding space. And according to Table~\ref{tab_all}, we note that DeepKmeans achieve the best clustering accuracy, which indicates the significant advantage of DeepKmeans.

\subsection{Running Time Comparison}
We compare the running time of DeepKmeans, DEC and DCEC on the benchmark datasets, including MNIST, USPS, COIL-20, and FRGC. For DeepKmeans, we stop the clustering process when there are less than 0.1\% of samples than change their clustering assignments between two consecutive iterations.
\begin{figure}[htbp]
	\centerline{\includegraphics{img/runningtime}}
	\caption{Running time comparisons of DeepKmeans, DEC and DCEC.}
	\label{fig_time}
\end{figure}

Fig.~\ref{fig_time} shows the running time of each method. For small dataset COIL-20, the running time of each method is close. For large datasets, e.g., MNIST, DeepKmeans takes a longer but acceptable time than DEC and DCEC. The increase in the running time is due to the eigen-decomposition of $\mathbf{S}_w$. Integrating with approximate methods such as power iteration and Lanczos algorithm, the running time will be reduced. We leave this for a future work.

